Identity Overlap Between Face Recognition Train/Test Data: Causing Optimistic Bias in Accuracy Measurement

A fundamental tenet of pattern recognition is that overlap between training and testing sets causes an optimistic accuracy estimate. Deep CNNs for face recognition are trained for N-way classification of the identities in the training set. Accuracy is commonly estimated as average 10-fold classification accuracy on image pairs from test sets such as LFW, CALFW, CPLFW, CFP-FP and AgeDB-30. Because train and test sets have been independently assembled, images and identities in any given test set may also be present in any given training set. In particular, our experiments reveal a surprising degree of identity and image overlap between the LFW family of test sets and the MS1MV2 training set. Our experiments also reveal identity label noise in MS1MV2. We compare accuracy achieved with same-size MS1MV2 subsets that are identity-disjoint and not identity-disjoint with LFW, to reveal the size of the optimistic bias. Using more challenging test sets from the LFW family, we find that the size of the optimistic bias is larger for more challenging test sets. Our results highlight the lack of and the need for identity-disjoint train and test methodology in face recognition research.

==> figures/supp_mat/cplfw-no-face.tex <==
\begin{figure}[h]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{1\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0034/34_1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0041/41_2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0056/56_1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0128/128_2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0148/148_2.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0149/149_2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0164/164_2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0178/178_2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0196/196_1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/cplfw-no-face/0198/198_2.jpg}
            \end{subfigure}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of no-face images in the CPLFW .bin file.}
\label{fig:no-face}
\end{figure}

==> figures/supp_mat/one-matches-many.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5881007/5.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5881007/6.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5881007/7.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5881007/8.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5881007/9.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5864520/10.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5864520/11.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5864520/12.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5864520/13.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/0/0_5864520/14.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5881007, 0\_5864520}
        \end{subfigure}
        
        \begin{subfigure}[b]{\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5871953/0.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5871953/1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5871953/2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5871953/3.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5871953/4.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5873714/0.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5873714/1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5873714/2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5873714/3.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5873714/4.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5887689/8.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5887689/9.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5887689/11.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5887689/17.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/1/0_5887689/20.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5871953, 0\_5873714, 0\_5887689}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of identity mis-categorization in MS1MV2. Each row shows the images in a folder (identity).}
\label{fig:one-match-many-1}
\end{figure}



\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836779/1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836779/2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836779/3.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836779/4.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836779/5.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836940/5.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836940/6.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836940/7.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836940/8.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5836940/9.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5885967/5.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5885967/6.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5885967/7.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5885967/8.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/4/0_5885967/9.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5836779, 0\_5836940, 0\_5885967}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5851833/4.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5851833/5.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5851833/6.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5851833/7.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5851833/8.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5891595/15.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5891595/16.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5891595/17.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5891595/18.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5891595/19.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5904682/0.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5904682/1.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5904682/2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5904682/3.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/5/0_5904682/4.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5851833, 0\_5891595, 0\_5904682}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of identity mis-categorization in MS1MV2. Each row shows the images in a folder (identity).}
\label{fig:one-match-many-2}
\end{figure*}


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5845667/13.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5845667/14.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5845667/17.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5845667/19.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5845667/22.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5883590/31.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5883590/32.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5883590/33.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5883590/54.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5883590/58.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5903985/2.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5903985/3.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5903985/4.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5903985/5.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/6/0_5903985/6.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5845667, 0\_5883590, 0\_5903985}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5823820/9.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5823820/10.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5823820/11.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5823820/12.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5823820/13.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5844082/53.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5844082/54.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5844082/55.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5844082/56.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5844082/57.jpg}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5877124/37.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5877124/38.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5877124/39.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5877124/40.jpg}
            \end{subfigure}
            \begin{subfigure}[b]{0.19\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/one-matches-many/10/0_5877124/41.jpg}
            \end{subfigure}
            \caption{Images at folder: 0\_5823820, 0\_5844082, 0\_5877124}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of identity mis-categorization in MS1MV2. Each row shows the images in a folder (identity).}
\label{fig:one-match-many-3}
\end{figure*}

==> figures/supp_mat/same_identity.tex <==
\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{0.9\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/0/1715_0.jpg}
                \caption{Naoto\_Kan\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/0/82.jpg}
                \caption{0\_5858920/82}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/1/2837_0.jpg}
                \caption{Drew\_Gooden\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/1/25.jpg}
                \caption{0\_5870377/25}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/2/2643_1.jpg}
                \caption{Rick\_Pitino\_4}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/2/40.jpg}
                \caption{0\_5859710/40}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/3/1966_0.jpg}
                \caption{Luiz\_Inacio\_Lula\_da\_Silva\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/3/64.jpg}
                \caption{0\_5835410/64}
            \end{subfigure}
        \end{subfigure}

        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/4/2322_1.jpg}
                \caption{Richard\_Chamberlain\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/4/3.jpg}
                \caption{0\_5867244/3}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/5/2658_1.jpg}
                \caption{Rudolph\_Giuliani\_20}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/5/79.jpg}
                \caption{0\_5827623/79}
            \end{subfigure}       
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/6/1883_1.jpg}
                \caption{Heizo\_Takenaka\_7}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/6/6.jpg}
                \caption{0\_5880926/6}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/7/2481_0.jpg}
                \caption{Elena\_Bovina\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/7/98.jpg}
                \caption{0\_5898207/98}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/8/242_1.jpg}
                \caption{Mike\_Krzyzewski\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/8/46.jpg}
                \caption{0\_5846710/46}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/9/1796_0.jpg}
                \caption{Steve\_Valentine\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/9/72.jpg}
                \caption{0\_5879521/72}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the same identity occur in both LFW and MS1MV2. 
   }
\label{fig:same-identity-1}
\end{figure*}


\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{0.9\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/10/2227_1.jpg}
                \caption{Julianne\_Moore\_15}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/10/82.jpg}
                \caption{0\_5837950/82}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/11/1542_1.jpg}
                \caption{Condoleezza\_Rice\_5}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/11/91.jpg}
                \caption{0\_5835176/91}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/12/2905_0.jpg}
                \caption{Maria\_Shriver\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/12/68.jpg}
                \caption{0\_5842997/68}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/13/2312_1.jpg}
                \caption{Nancy\_Pelosi\_9}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/13/106.jpg}
                \caption{0\_5885609/106}
            \end{subfigure}
        \end{subfigure}

        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/14/1101_1.jpg}
                \caption{Paul\_Burrell\_10}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/14/33.jpg}
                \caption{0\_5834783/33}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/15/1978_0.jpg}
                \caption{Mark\_Philippoussis\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/15/21.jpg}
                \caption{0\_5839025/21}
            \end{subfigure}       
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/16/553_1.jpg}
                \caption{Silvio\_Berlusconi\_32}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/16/33.jpg}
                \caption{0\_5882840/33}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/17/741_1.jpg}
                \caption{Keanu\_Reeves\_7}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/17/110.jpg}
                \caption{0\_5865903/110}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/18/2055_1.jpg}
                \caption{Sam\_Torrance\_3}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/18/14.jpg}
                \caption{0\_5880918/14}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/19/2803_1.jpg}
                \caption{George\_W\_Bush\_150}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_identity/19/34.jpg}
                \caption{0\_5841527/34}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the same identity occur in both LFW and MS1MV2. 
   }
\label{fig:same-identity-2}
\end{figure*}

==> figures/supp_mat/same_images.tex <==
\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{0.9\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/0/1891_0.jpg}
                \caption{Craig\_Burley\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/0/57.jpg}
                \caption{0\_5890009/57}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/1/2434_0.jpg}
                \caption{Benazir\_Bhutto\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/1/26.jpg}
                \caption{0\_5836537/26}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/2/2216_1.jpg}
                \caption{Johnny\_Unitas\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/2/23.jpg}
                \caption{0\_5856661/23}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/3/410_1.jpg}
                \caption{Doug\_Moe\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/3/6.jpg}
                \caption{0\_5872926/6}
            \end{subfigure}
        \end{subfigure}

        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/4/2011_0.jpg}
                \caption{Johnny\_Depp\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/4/67.jpg}
                \caption{0\_5892154/67}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/5/1550_1.jpg}
                \caption{Cruz\_Bustamante\_4}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/5/21.jpg}
                \caption{0\_5840766/21}
            \end{subfigure}       
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/6/1713_0.jpg}
                \caption{Nancy\_Reagan\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/6/26.jpg}
                \caption{0\_5874109/26}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/7/654_0.jpg}
                \caption{Barry\_Bonds\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/7/19.jpg}
                \caption{0\_5836919/19}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/8/1016_0.jpg}
                \caption{David\_McKiernan\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/8/3.jpg}
                \caption{0\_5897287/3}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/9/64_1.jpg}
                \caption{Nong\_Duc\_Manh\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/9/40.jpg}
                \caption{0\_5836715/40}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the same images occur in both LFW and MS1MV2. 
   }
\label{fig:same-image-1}
\end{figure*}


\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{0.9\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/10/1007_0.jpg}
                \caption{James\_Gandolfini\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/10/22.jpg}
                \caption{0\_5854640/22}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/11/319_1.jpg}
                \caption{Doug\_Moe\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/11/0.jpg}
                \caption{0\_5872926/0}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/12/2884_0.jpg}
                \caption{Leonid\_Kuchma\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/12/57.jpg}
                \caption{0\_5844623/57}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/13/720_1.jpg}
                \caption{Jerry\_Springer\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/13/102.jpg}
                \caption{0\_5841902/102}
            \end{subfigure}
        \end{subfigure}

        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/14/2193_0.jpg}
                \caption{Ilan\_Ramon\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/14/65.jpg}
                \caption{0\_5835892/65}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/15/912_0.jpg}
                \caption{Alex\_Barros\_2}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/15/5.jpg}
                \caption{0\_5883749/5}
            \end{subfigure}       
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/16/1644_0.jpg}
                \caption{Jeff\_Van\_Gundy\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/16/6.jpg}
                \caption{0\_5879676/6}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/17/2643_0.jpg}
                \caption{Rick\_Pitino\_3}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/17/8.jpg}
                \caption{0\_5859710/8}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/18/2929_1.jpg}
                \caption{Teddy\_Kollek\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/18/31.jpg}
                \caption{0\_5860410/31}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/19/1706_0.jpg}
                \caption{Jeane\_Kirkpatrick\_1}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\linewidth}
                \includegraphics[width=\linewidth]{images/supp-mat/same_image/19/13.jpg}
                \caption{0\_5837214/13}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the same image occur in both LFW and MS1MV2. 
   }
\label{fig:same-image-2}
\end{figure*}

==> table/cplfw-curation.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
         & CosFace & SphereFace & ArcFace & CurricularFace & MagFace & AdaFace \\ \hline
Original & 93.25   & 92.67      & 93.35   & 92.95          & 92.67   & 93.05   \\ \hline
Updated  & 95.04   & 94.56      & 95.12   & 94.72          & 94.72   & 94.82   \\ \hline
diff  & 1.79   & 1.89      & 1.77   & 1.77          & 2.05   & 1.77   \\ \hline
\end{tabular}
\caption{Performance of SOTA models on the updated CPLFW.}
\label{tab:cplfw-curate}
\end{table}
